Building Autocorrelation-Aware Representations for Fine-Scale Spatiotemporal Prediction

Many scientific prediction problems have spatiotemporal data- and modeling-related challenges in handling complex variations in space and time using only sparse and unevenly distributed observations. This paper presents a novel deep learning architecture, Deep learning predictions for LocATion-dependent Time-sEries data (DeepLATTE), that explicitly incorporates theories of spatial statistics into neural networks to address these challenges. In addition to a feature selection module and a spatiotemporal learning module, DeepLATTE contains an autocorrelation-guided semi-supervised learning strategy to enforce both local autocorrelation patterns and global autocorrelation trends of the predictions in the learned spatiotemporal embedding space to be consistent with the observed data, overcoming the limitation of sparse and unevenly distributed observations. During the training process, both supervised and semi-supervised losses guide the updates of the entire network to: 1) prevent overfitting, 2) refine feature selection, 3) learn useful spatiotemporal representations, and 4) improve overall prediction. We conduct a demonstration of DeepLATTE using publicly available data for an important public health topic, air quality prediction, in a well-studied, complex physical environment - Los Angeles. The experiment demonstrates that the proposed approach provides accurate fine-spatial-scale air quality predictions and reveals the critical environmental factors affecting the results.

==> review.tex <==
Review 1:
*1. Details of section II.B are sparse, why $X\_sp$ size is same as X, when several features are forced to be Zero. So, it’s not clear what the input size should be to the Encoder/Decoder layer.
*2. Paper is lacking ablation studies, details on how hyperparameters are set
*3. Page 7, second para: sentences 4 and 5 seems to be contradicting each other. (Done)
*4. In the absence of code, it would be extremely difficult for the results to be reproduced. 
Review 2:
*1. The parameters used in the baseline techniques are not shown. These parameters should be described, and the author(s) should state how the parameter tuning was done
?2. The architecture of the conv-LSTM should be better described (e.g., by using figures and tables to show the layers and parameters). 
*3. The author(s) stated the sources of the used data without providing a citation/link to those sources. (Done)
*4. Figure 5 and its caption do not match. (Done)
*5. Releasing publicly the used dataset would be good. (Done)

Review 3:
*1. The model is only evaluated on air pollution (PM2.5). It would be more convincing if the model is evaluated on other datasets or other spatiotemporal prediction tasks. (Future work)
*2. There are four parameters in the cost function (6). A parameter sensitivity analysis is needed to show the impact of these parameters.
3. The evaluation metric $R^2$ should be explained. (Done)


==> sections/archive.tex <==
In air quality prediction, typical sources of PM$_{2.5}$ measurements include: 1)~remote sensing (satellite) measurements, which can provide daily, near-global coverage but are limited in that they do not directly represent ground-level concentrations of PM$_{2.5}$, requiring converting optical measures to a mass concentration. Furthermore, these data typically suffer from a high percentage of missing observations~\citep{kloog2014new}; 2)~ambient monitoring with gravimetric and beta-attenuation instruments, which provide high-quality measurements but are expensive to operate. As a result, the spatial distribution of such devices is usually sparse. For example, in the Los Angeles metropolitan area, the U.S. Environmental Protection Agency (US EPA) sets only nine monitoring stations (red stars in Figure~\ref{Figure: Los Angeles EPA Sensor Locations}); 3)~mobile monitoring platforms (e.g., Google Street View cars) can be equipped with air quality sensors to collect street-level concentrations over large areas, but fleets are limited, and the data are not pervasive or accessible to the public; 4) low-cost sensors, such as PurpleAir,\footnote{https://www2.purpleair.com/} provide a more widespread network that captures finer spatial and temporal variability than Federal- and State-operated monitoring networks ~\citep{cavaliere2018development}. Compared to the EPA monitoring stations, there are about 150 active PurpleAir sensors (purple dots in Figure~\ref{Figure: Los Angeles EPA Sensor Locations}) in the same area during November 2018. However, the spatial coverage still does not satisfy the needs of studies that require close tracking of exposure-response relationships (e.g., \cite{murray2006study}). 

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.95\columnwidth]{figures/epa_sensor_locations.jpg}
  \caption{Red stars represent the locations of the EPA monitoring stations in the Los Angeles metropolitan area (more than 250km$^2$ per station). Blue dots represent the locations of PurpleAir sensors in the same region. The approximate geographical area size of the displayed map is 50km$\times$40km.}
  \label{Figure: Los Angeles EPA Sensor Locations}  
\end{figure}

This paper proposes a deep learning architecture for fine-scale predictions of location-dependent time series data and applies the approach for air quality prediction using publicly available and easily accessible Web data, including geographic data for describing the nature and built environment from OpenStreetMap (OSM),\footnote{https://www.openstreetmap.org/} air quality data from PurpleAir, and meteorological data from DarkSky.\footnote{https://darksky.net/dev} These data either have global coverage (OSM and DarkSky) or alternative data exist in many places (e.g.,AirBox for air quality data from low-cost sensors~\citep{chen2017airbox}). Predicting air quality using Web data that have global coverage or are easily substituted with other similar data has the advantage that the same approach can apply to many places without retooling the architecture to accommodate the availability of a dataset. For example, air quality data from ambient monitoring sites and low-cost sensors are usually available online and easy to access while remote sensing data and street view data are proprietary, which are sometimes costly and challenging to obtain. 


% We denote ``dynamic data'' as the features changing along the time. Our system up-scales the weather data using cubic interpolation method if the target resolution is higher than the given meteorological data. 
% Our model takes time information (i.e., hour of a day and day of a week) as additional dynamic features.

\subsubsection{Static Grid Data}
We define ``static data'' as constant features like the built environment and topography. 
Our approach generates a feature vector to describe various types of built environments. Figure \ref{figure:Geographic Feature Construction} provides an example of roads (line feature) and land uses (polygon feature) in cell ``A''. 
For line features, our approach sums up lengths of various types in the cell. Cell A contains 450m pedestrian and 1,030m motorway, which forms a vector as [450, 1,030]. Figure \ref{figure:Gridded Primary Road} shows the length of primary roads in Los Angeles on a grid map. There are hot spots in the Downtown LA and at some intersections.
Similar to the polygon features, we compute the sum of the areas. There are 50,000m$^2$ green lands and 15,000m$^2$ industrial areas in cell A, represented as [50,000, 15,000]. 
Our model adds topographic features (i.e., coordinate) to indicate location information. Therefore, the entire static feature vector for cell A is constructed as [450, 1,030, 50,000, 15,000, longitude, latitude]. 

\begin{figure}[h]
\centering
    \subfigure[Example of cell A]{
        \begin{minipage}[t]{0.47\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{figures/gridded_geo_features.jpg}
            \label{figure:Geographic Feature Construction}
        \end{minipage}
    }
    \subfigure[Grid primary roads]{
        \begin{minipage}[t]{0.47\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{figures/gridded_primary_road.jpg}
            \label{figure:Gridded Primary Road}
        \end{minipage}
    }
\caption{(a) shows an example roads and land uses with various types in a 500m$\times$500m cell. (b) shows the length of primary roads on the same grid map as Figure 2. The darker the color, the more primary roads in the cell. The uncolored cells do not contain value inside.}
\end{figure}


% Due to the relatively small cell size in the fine-scale prediction task, the proposed architecture employs a spatial constraint assuming air quality values at close spatial distance tend to be similar. The proposed architecture applies the following semi-supervised cost function on the predictions (of both labeled and unlabeled locations) to force nearby cell values to be similar:

% \begin{equation}
% L_{sc} = {\sum_{i=1}^{n} \sum_{k=1}^{K}\sum_{j \in {N_{k_i}}} e^{-k}\bar{L}(p_i, p_j)} 
% \label{Equation: Spatial Constraint}
% \end{equation}

% \noindent where $n$ is the number of total cells, $K$ is the number of neighboring steps, ${N_{k_i}}$ is the neighboring cells of cell $i$ within step $k$, and $\bar L$ is the loss function with MSE. 

% In general, the model first utilizes a sparse layer to select air-quality-related features and remove irrelevant ones. Then, the model uses a pretrained auto-encoder to learn the latent embedding of the inputs. Afterwards, the output representations are served as the inputs to the Conv-LSTM layers. The Conv-LSTM layers jointly learn the spatiotemporal effects with multiple kernel sizes. By adding the spatial constraint, the model leverages the unlabeled cells during the training process. Finally, 


In practice, the model learns useful information from the combination of the current latent embedding (i.e., the interactive effects) of the selected features from neighbors and the previous hidden memory in the Conv-LSTM Cell (Figure~\ref{Figure: Whole Structure}). The Conv-LSTM operation replaces the internal matrix multiplications of the original LSTM with convolution operations using the following equations: \todo{modify this using our parameters}

\begin{displaymath}
        \boldsymbol{i}^{(t)}= \sigma(\boldsymbol{W_i}\odot[\boldsymbol{X}^{(t)}, \boldsymbol{H}^{(t-1)}] + \boldsymbol{b_i})
\end{displaymath}
\begin{displaymath}
        \boldsymbol{f}^{(t)}= \sigma(\boldsymbol{W_f}\odot[\boldsymbol{X}^{(t)}, \boldsymbol{H}^{(t-1)}] + \boldsymbol{b_f})
\end{displaymath}
\begin{displaymath}
    \boldsymbol{\widetilde{C}}^{(t)} = \tanh(\boldsymbol{W_C}\odot[\boldsymbol{X}^{(t)}, \boldsymbol{H}^{(t-1)}] + \boldsymbol{b_C})
\end{displaymath}
\begin{displaymath}
         \boldsymbol{C}^{(t)} = \boldsymbol{f}^{(t)} \times \boldsymbol{C}^{(t-1)}+\boldsymbol{i}^{(t)} \times \boldsymbol{\widetilde{C}}^{(t)}
\end{displaymath}
\begin{displaymath}
        \boldsymbol{o}^{(t)}= \sigma(\boldsymbol{W_o}\odot[\boldsymbol{X}^{(t)}, \boldsymbol{H}^{(t-1)}] + \boldsymbol{b_o})
\end{displaymath}
\begin{displaymath}
        \boldsymbol{h}^{(t)}= \boldsymbol{o}^{(t)} \times \tanh{\boldsymbol{C}^{(t)}}
\end{displaymath}

\noindent where $\boldsymbol{i}$, $\boldsymbol{f}$, $\boldsymbol{C}$, and $\boldsymbol{o}$ correspond to the input gate, forget gate, memory cell, and output gate in the LSTM, respectively; $\boldsymbol{X}^{(t)}$ is the current input, and $\boldsymbol{H}^{(t-1)}$ is the last output; $\odot$ denotes the convolution operation, $\times$ is the element-wised multiplication; $\boldsymbol{W}$ terms denote the weight matrices, and $\boldsymbol{b}$ terms are the bias vectors. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Data Preprocessing} 
% In practical, the low-cost sensors might suffer from exceptional events such as disconnection to the network or improper installations, so the sensor data generally contain missing values and outliers. Thus, our first step is data preprocessing for the PurpleAir $PM_{2.5}$ data. Typically, there are two kinds of outliers in the PurpleAir PM$_{2.5}$ observations. First, the sensors that provide extremely large numbers (more than 5000$\mu$g/m$^3$) (Figure \ref{Figure: Extremely Large Numbers}) are removed since it is not possible to achieve this large number in $PM_{2.5}$ concentrations. We suspect them as equipment malfunction. Second, there are extremely small numbers with tiny but frequent vibrations in the observations (Figure \ref{Figure: Extremely Small Numbers}). We consider these sensors as outliers because they do not provide useful information (values) in a reasonable range. We guess these sensors might be wrongly labeled as ``indoor sensors''. Table \ref{Table: Details of Datasets} shows the details about the air quality datasets with different resolutions we use in the experiment after mapping the sensor data to the grids. 

% \begin{figure}[h]
% \centering
%     \subfigure[Extremely large numbers in PM$_{2.5}$ observations]{
%         \begin{minipage}[t]{0.95\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/outlier1.jpg}
%             \label{Figure: Extremely Large Numbers}  
%         \end{minipage}
%         }
%     \subfigure[Extremely small numbers in PM$_{2.5}$ observations]{
%     \begin{minipage}[t]{0.95\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/outlier2.jpg}
%         \label{Figure: Extremely Small Numbers}  
%     \end{minipage}
%     }
% \centering
% \caption{Two kinds of outliers in the PurpleAir PM$_{2.5}$ observations and the corresponding sensors will be removed from the training and testing process}
% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[h]
% \centering
% \caption{Comparison between our model and the baselines}
% \label{Table: RMSE Results}
% \renewcommand\arraystretch{1.1}
% \begin{tabular}{c|| c | c c c c c c c c c}
%      & {Metric} & RF & IDW & OK & U-Air & DeepAir & C-LSTM & D-LATTE-V1 & D-LATTE-V2 & DeepLATTE \\ \hline\hline
%     \multirow{2}{*}{Jan.18} & RMSE & 8.48 & 0.76 & & & & & & & 6.57
%                             \\ & R2 & 0.76 & 0.76 & & & & & & & 0.83 \\ \hline
%     \multirow{2}{*}{Apr.18} & RMSE & 4.32 & 4.37 & & & & & & &
%                             \\ & R2 & 0.85 & 0.85 & & & & & & \\ \hline
%     \multirow{2}{*}{Jul.18} & RMSE & 3.50 & 3.67 & & & & 5.49 & 4.02 & 3.49 & 3.42
%                             \\ & R2 & 0.86 & 0.85 & & & & 0.65 & 0.80 & & 0.87 \\ \hline
%     \multirow{2}{*}{Oct.18} & RMSE & 4.47 & 4.37 & & & & 6.11 & 5.67 & 5.29 & 4.17
%                             \\ & R2 & 0.90 & 0.91 & & & & 0.82 & 0.85 & 0.86 & 0.91 \\ \hline
%     \multirow{2}{*}{Jan.19} & RMSE & 8.58 & 8.48 & & & & & & & 6.57
%                             \\ & R2 & 8.58 & 8.48 & & & & & & & 0.83 \\ \hline
%     \multirow{2}{*}{Apr.19} & RMSE & 8.58 & 8.48 & & & & & & &
%                             \\ & R2 & 8.58 & 8.48 & & & & & &  &\\ \hline
%     \multirow{2}{*}{Jul.19} & RMSE & 8.58 & 8.48 & & & & & & &
%                             \\ & R2 & 8.58 & 8.48 & & & & & &  &\\ \hline
%     \multirow{2}{*}{Oct.19} & RMSE & 8.58 & 8.48 & & & & & & &
%                             \\ & R2 & 8.58 & 8.48 & & & & & &  &\\ \hline
    
    % \textbf{Method} & \textbf{RMSE} & \textbf{R2} & \textbf{RMSE} & \textbf{R2} \\ \hline
    % RF & 14.184 & 0.739 & 14.424 & 0.729 \\ \hline
    % IDW & 9.851 & 0.872 & 10.754 & 0.847 \\ \hline
    % LSTM & 15.620 & 0.630 & 15.032 & 0.641 \\ \hline
    % Conv-LSTM & 11.586 & 0.775 & 11.303 & 0.837 \\ \hline
    % Our Model & \textbf{9.704} & \textbf{0.876} & \textbf{10.256} & \textbf{0.861} \\ \hline
%     \end{tabular}
% \end{table*}

% \begin{table}[h]
% \centering
% \caption{Details of PM$_{2.5}$ grid data}
% \label{Table: Details of Datasets}
% \begin{tabular}{ c | c | c }
% \hline
%     \textbf{Resolution} & \textbf{500m$\times$500m} & \textbf{1,000m$\times$1,000m} \\ \hline
%     Number of Labels & 138 & 126 \\ \hline
%     Number of Grids & 6,992 & 1,748 \\ \hline
%     PM$_{2.5}$ Average& 25.99 & 26.01 \\ \hline
%     PM$_{2.5}$ STD.& 27.40 & 27.38 \\ \hline
% \end{tabular}
% \end{table}


\begin{figure}[htbp]
\centering
    \subfigure[Morning, 5AM to 12PM]{
        \begin{minipage}[t]{0.46\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/feb19_m.png}
            % \vspace{-.1in}
            \label{figure: feb19_m}
        \end{minipage}
    }
    \subfigure[Afternoon, 12PM to 5PM]{
        \begin{minipage}[t]{0.46\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/feb19_a.png}
            % \vspace{-.1in}
            \label{figures: feb19_a}
        \end{minipage}
    }
    \vspace{.1in}
    \subfigure[Evening, 5PM to 9PM]{
        \begin{minipage}[t]{0.46\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/feb19_e.png}
            % \vspace{-.1in}
            \label{figure: feb19_e}
        \end{minipage}
    }
    \subfigure[Night, 9PM to 5AM]{
        \begin{minipage}[t]{0.46\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/feb19_n.png}
            % \vspace{-.1in}
            \label{figures: feb19_n}
        \end{minipage}
    }
\caption{Daily pattern of the predictions from DeepLATTE}
\end{figure}
